Maximum cut on interval graphs of interval count four is NP-complete

The computational complexity of the MaxCut problem restricted to interval graphs has been open since the 80's, being one of the problems proposed by Johnson on his Ongoing Guide to NP-completeness, and has been settled as NP-complete only recently by Adhikary, Bose, Mukherjee and Roy. On the other hand, many flawed proofs of polynomiality for MaxCut on the more restrictive class of unit/proper interval graphs (or graphs with interval count 1) have been presented along the years, and the classification of the problem is still unknown. In this paper, we present the first NP-completeness proof for MaxCut when restricted to interval graphs with bounded interval count, namely graphs with interval count 4.

==> intervalcount.tex <==
\definecolor{myblue}{RGB}{0,0,255}
\definecolor{mygreen}{RGB}{31,120,68}
\definecolor{mygrey}{RGB}{156, 156, 156}
\definecolor{darkblue}{RGB}{0, 0, 153}



\def\epsilon{0.02} %use to define the open intervals
\def\n{4}
\def\m{1}
\def\h{3}
\def\hprime{4}
\def\t{4*\n}

\begin{figure}[thb]
  \begin{center}
      \resizebox{\textwidth}{!}{
        \begin{tikzpicture}[scale=1.0]
        
          \pgfsetlinewidth{1pt}
          \tikzset{thinScale/.style={dash pattern=on 1pt off 2pt, line width=0.5\pgflinewidth, mygrey}}
          \tikzset{thickScale/.style={dash pattern=on 2.5pt off 3pt, line width=2.0pt}}
          \tikzset{closeInterval/.style={{|[scale=0.8,width=6.8,line width=1.0pt, sep=-0.50pt]}-{|[scale=0.8,width=6.8,line width=1.0pt,sep=-0.50pt]}, line width=2pt}}
          \tikzset{shortInterval/.style={dot diameter=1.4pt, dot spacing=1.9pt, dots}}



          %Scale
          \foreach \i in {1, ..., \n} {
            \foreach \j in {0, ..., \m}{
              \draw[thinScale] (2*\i-2 + \t*\j,0)--(2*\i-2 + \t*\j,-\n - 1);
              \draw[thinScale] (2*\i-1.5 + \t*\j,0)--(2*\i-1.5 + \t*\j,-\n - 1);
              \draw[thinScale] (2*\i-1 + \t*\j,0)--(2*\i-1 + \t*\j,-\n - 1);
            }
          }

          \draw[thinScale] (2*\n,0)--(2*\n,-\n - 1) (2*\h + 2*\n-2,0)--(2*\h + 2*\n-2,-\n - 1) (2*\hprime + 2*\n-2,0)--(2*\hprime + 2*\n-2,-\n - 1) (4*\n-1,0)--(4*\n-1,-\n - 1) (4*\n-0.5,0)--(4*\n-0.5,-\n - 1);
          % \draw[thickScale] (0,0)--(0,-5);
          % \draw[thickScale] (8*\n-2,0)--(8*\n-2,-5);
          \draw[thickScale, mygreen] (\t,0)--(\t,-5);


          \foreach \i in {1, ..., \n}{
            \foreach \j in {0, ..., \m}{

               %left short intervals
               \draw[shortInterval] (2*\i-2+\epsilon + \t*\j,-\i+0.1)--(2*\i-1.5 + \t*\j-\epsilon,-\i+0.1); 

               %right short intervals
               \draw[shortInterval] (2*\i-1.5+\epsilon + \t*\j,-\i-0.1)--(2*\i-1 + \t*\j-\epsilon,-\i-0.1); 

               %left long intervalss
               \draw[closeInterval,red] (2*\i-2 + \t*\j,-\i)--(2*\i-1.5 + \t*\j,-\i);

               %right long intervals
               \draw[closeInterval,red] (2*\i-1.5 + \t*\j,-\i-0.2)--(2*\i-1 + \t*\j,-\i-0.2); 
            }

            %link intervals
            \draw[closeInterval,orange] (2*\i-1,-\i-0.6)--({2*(\i-1)+ 4*\n},-\i-0.6); 

          }


          %intervals C1 and C2
          \draw[closeInterval,myblue] (2*\h-1,-\h-0.4)--(2*\h + 2*\n-2,-\h-0.4);

          %intervals C3 and C4
          \draw[closeInterval,myblue] (2*\hprime-1, -\hprime-0.4)--(2*\hprime + 2*\n-2,-\hprime-0.4); 

          %left long intervals of E1
          \draw[closeInterval,myblue]  (2*\n,-0.4)--(4*\n-1,-0.4); 


          % left short intervals of E1
          \draw[shortInterval] (2*\h + 2*\n - 2 + \epsilon,-0.2)--(2*\hprime + 2*\n - 2 - \epsilon,-0.2);


          %right long intervals of E1
          \draw[closeInterval,red] (4*\n - 1,-0.6)--(4*\n - 0.5,-0.6); 

          %right short intervals of E1
          \draw[shortInterval] (4*\n - 1 + \epsilon,-0.5)--(4*\n - 0.5 - \epsilon,-0.5);

      \end{tikzpicture}
    }
    \caption{The closed intervals in ${\cal S}_1\cup \bigcup_{i=1}^4{\cal H}^{2}_i$ of a graph on 4 vertices. We consider $e_1$ to be equal to $v_3v_4$. Each colour represents a different interval size. 
   %%%% The short intervals are contained in the dotted (open) intervals.
   The short intervals are represented by the dots located inside the open (red) intervals.
   Vertical lines mark the endpoints of the intervals in ${\cal S}_1\cup \bigcup_{i=1}^4{\cal H}^{2}_i$,
   % Vertical lines before the green vertical line mark the endpoints of the intervals in 
   % ${\cal S}_1\setminus \Lambda$,
 %%   ${\cal S}_1\setminus {\cal L}$, 
    while the green vertical line marks the beginning of the intervals in ${\cal S}_2$.}\label{fig:intervalCount}
  \end{center}
\end{figure}

